Towards Flexible Visual Relationship Segmentation

Visual relationship understanding has been studied separately in human-object interaction(HOI) detection, scene graph generation(SGG), and referring relationships(RR) tasks. Given the complexity and interconnectedness of these tasks, it is crucial to have a flexible framework that can effectively address these tasks in a cohesive manner. In this work, we propose FleVRS, a single model that seamlessly integrates the above three aspects in standard and promptable visual relationship segmentation, and further possesses the capability for open-vocabulary segmentation to adapt to novel scenarios. FleVRS leverages the synergy between text and image modalities, to ground various types of relationships from images and use textual features from vision-language models to visual conceptual understanding. Empirical validation across various datasets demonstrates that our framework outperforms existing models in standard, promptable, and open-vocabulary tasks, e.g., +1.9 $mAP$ on HICO-DET, +11.4 $Acc$ on VRD, +4.7 $mAP$ on unseen HICO-DET. Our FleVRS represents a significant step towards a more intuitive, comprehensive, and scalable understanding of visual relationships.

==> preamble.tex <==
\usepackage{float}
\usepackage{amsmath}

\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\todo}[1]{{\color{red}#1}}
\newcommand{\TODO}[1]{\textbf{\color{red}[TODO: #1]}}

\newcommand\blfootnote[1]{%
  \begingroup
  \renewcommand\thefootnote{}\footnote{#1}%
  \addtocounter{footnote}{-1}%
  \endgroup
}

\newcommand{\modelname}{\emph{SwapAnything}}
\newcommand{\editbooth}{\emph{EditBooth}}

\newcommand{\bs}[1]{{\boldsymbol{#1}}}
\newcommand{\getNoise}{\bs{\epsilon}_{\theta^*}}
\newcommand{\depsh}{\bs{\hat{\epsilon}}_\theta}
\newcommand{\prompt}[1]{``\emph{#1}"}

\newcommand{\z}{\mathbf{z}}
\newcommand{\x}{\mathbf{x}}
\newcommand{\cond}{\mathbf{c}}
\newcommand{\sigm}{\mathbf{\sigma}}
\newcommand{\eps}{\mathbf{\epsilon}}
\newcommand{\mask}{\mathbf{M_{src}}}


\newcommand{\selfoutput}{$\bs{\phi}$}
\newcommand{\selfmap}{$\bs{A}$}
\newcommand{\crossmap}{$\bs{\phi}$}
\newcommand{\imagelatent}{$\bs{z}$}

